GLoRE: Evaluating Logical Reasoning of Large Language Models

Large language models (LLMs) have shown significant general language understanding abilities. However, there has been a scarcity of attempts to assess the logical reasoning capacities of these LLMs, an essential facet of natural language understanding. To encourage further investigation in this area, we introduce GLoRE, a General Logical Reasoning Evaluation platform that not only consolidates diverse datasets but also standardizes them into a unified format suitable for evaluating large language models across zero-shot and few-shot scenarios. Our experimental results show that compared to the performance of humans and supervised fine-tuning models, the logical reasoning capabilities of large reasoning models, such as OpenAI's o1 mini, DeepSeek R1 and QwQ-32B, have seen remarkable improvements, with QwQ-32B achieving the highest benchmark performance to date. GLoRE is designed as a living project that continuously integrates new datasets and models, facilitating robust and comparative assessments of model performance in both commercial and Huggingface communities.

==> subtexs/4-method.tex <==
\section{Evaluation Methodology}

We evaluate open-sourced and closed LLMs (e.g., ChatGPT, GPT-4) across seven logical reasoning scenarios: \emph{zero-shot evaluation}, \emph{few-shot evaluation}, and \emph{instruction tuning evaluation}.

\noindent \textbf{Zero-shot Evaluation}
In this setup, task inputs are converted into prompts using templates, and gold labels are verbalized~\cite{liu2021pretrain}. LLMs generate the verbalized gold answer.
Prior research shows that ChatGPT may underperform in question-answering tasks without optimized instructions~\cite{zhong2023agieval}. To address this, we explored various zero-shot prompting methods to improve model performance.
Instructions are tailored to each dataset based on their target outputs. The finalized instructions for the three task types are integrated into GLoRE.

\noindent \textbf{Few-shot Evaluation}
\label{sec:in-context-method }
LLMs excel at in-context learning~\cite{dong2023survey}, where performance improves with context examples and demonstration methods~\cite{liu2021makes}. For this study, we randomly sampled instances (1 for 1-shot, 2 for 2-shot, and 5 for 5-shot) from each dataset and appended them to the prompt. We used the same model configuration as in the zero-shot scenario.

\noindent \textbf{Instruction Tuning}
\label{sec:tuning }
Open-sourced LLMs like LLaMA allow task-specific fine-tuning~\cite{wu2023pmc}, offering an advantage over closed models. We evaluate this by fine-tuning open-sourced LLMs using instruction-tuning, providing specific instructions for distinct tasks.

%We converted a specific logic reasoning training set into a instruction-prompting framework. 
%This process entailed reforming the dataset such that each instance was paired with a clear, directive instruction, an input, and a target output. We then fine-tuned an open-sourced LLM  with this transformed training dataset and the fine-tuning process. After instruction-tuning, we evaluate the model performance on the specific test set for the training task and the zero-shot performance on the other logic reasoning tasks to examine its cross-task generalization ability. 

%The primary objective of this evaluation was to assess the extent to which instruction-prompted fine-tuning could boost the model's performance on the logical reasoning task. 

%\subsection{Self-Consistency Evaluation}
%\label{sec:self-consistency}
%\input{subtexs/voting}
%In logical reasoning tasks, the model must grasp the connection between various facts or statements to make correct deductions. These tasks, by nature, demand a comprehensive understanding of the logical relations within the context rather than treating each piece of information in isolation. The validity of logical conclusions drawn from these tasks remains intact regardless of the sequence of facts or the specific structuring of sentences.

%To probe LLM's robustness in handling such tasks, we employed self-consistency probing, a technique useful for testing stability against minor context perturbations \cite{wang2023selfconsistency,jang2023consistency}.
%Figure~\ref{fig:consistency} shows the procedure, which involves creating $K$ unique contexts by randomly rearranging sentences from the original context, each then fed to LLM to generate an answer. The final response was chosen based on a majority vote.
\iffalse
\textbf{Chain-of-Thought Evaluation}
\label{sec:cot-method}
It has been shown that Chain-of-Thought (CoT) can improve the math \cite{imani2023mathprompter,chen2022program} and logic \cite{ling2023deductive} capabilities of LLMs.
We explore zero-shot CoT prompting~\cite{kojima2023large} on logical reasoning datasets. 
%The detailed settings are shown in Appendix~\ref{sec:appendix_b}.

%We add the prompt ``Let's think step by step'' to the instruction as shown in Appendix~\ref{sec:appendix_b}. By adding this prompt, LLM can generate longer reasoning texts exemplifying the reasoning steps. The final answer for each CoT reasoning process is collected by excluding the reasoning process.  
\fi

\input{tables/mainres}

%\subsection{Chat UI Based Evaluation}
%\label{sec:chat-ui-method}
%To complement the API-based evaluations, we also conducted manual tests within the GPT-4 chat UI. We use a separate Chat box for each task to query randomly sampled examples without leaking the answer. In this way, a stream of unlabeled examples can be gradually explored during the evaluation procedure. The manual test results provide an intriguing perspective on the GPT-4 model's performance in a chat-based user interface. This more interactive, dynamic environment provides a more realistic scenario reflecting how end-users might engage with the model in practice.

%\subsection{Evaluation of Generated Responses}

%Apart from the quantitative evaluation of model performance, we also evaluate the quality of models' generations. We explore human evaluation as well as automatic evaluation methods.
%We evaluate a model's generation in four aspects: {\it coherence}, {\it completeness}, {\it correctness}, and {\it relevance}. The score ranges from 1 to 5 with 1 indicating poor quality and 5 indicating excellent. The guidance to our evaluation metrics is detailed in Appendix~\ref{appendix_metrics}.

%The protocols are given to 3 outsourced annotators to score. They are assigned with the same evaluation set, so each sample is assigned with 3 scores to ensure reliability. We calculated the average scores and inter-annotator agreement using Cohen's Kappa to ensure consistency among annotators.

%Automatic evaluation of reasoning chains is an ongoing endeavor. Recently, \citet{prasad2023receval} used Natural Language Inference (NLI) to validate the correctness of reasoning chains. However, the method takes correctness as the main evaluation metric, leaving coherence, relevance, and completeness untouched.
%We conducted an experiment for automatically evaluating reasoning chains through ChatGPT. The evaluation of generated text using ChatGPT is a promising line of research. Building upon existing evaluation metrics, we guided ChatGPT to act as an evaluator of CoT. This involves showing the model with examples from our manually scored evaluations to ensure alignment. The prompt we use for this approach is detailed in Appendix~\ref{appendix_auto}.
%While this is an approximate method, it offers a more automated means of assessment and can complement human evaluations.


%\subsection{In-context Learning Evaluation}
%\label{sec:in-context-method}
%LLMs are capable of achieving efficient in-context learning \cite{dong2023survey}. Different from zero-shot evaluation, in this setup, $N$  examples with gold answers are used as the context for LLMs to infer the answer for a test query. Each example is converted to a prompt in the same way as the zero-shot evaluation, and all the prompts for the $N$ examples are concatenated together as the inputs in the final prompt. Different numbers of context examples and in-context demonstration methods \cite{liu2021makes} can lead to different results. In this study, we consider the basic random sampling strategy and leave the more sophisticated method for future work. 


==> subtexs/discussion.tex <==
\section{Discussion}
We provide a more analytical and investigative examination of the logical reasoning capabilities of large models like GPT-4.

\subsection{Zero-Shot Experiments on Various Types of Logical Reasoning Data}
    Our study is not limited to the presentation of datasets but includes an in-depth analysis of large models' performance across a diverse range of logical reasoning tasks. Notably, our zero-shot experiments revealed that large models like GPT-4 are highly sensitive to data distributions, resulting in significant performance variations across different datasets. This finding is crucial as it points to the need for more robust and adaptable models capable of consistent performance across various data distributions.
\subsection{Small-Sample Experiments Demonstrating Quick Adaptation}
    We have also conducted small-sample experiments which suggest that large models are effective tools for learning from small data samples. They demonstrate a rapid adaptation to the features of data distribution. This is a significant insight for future model training and fine-tuning, especially in scenarios where large datasets are not available or feasible.
\subsection{Chain of Thought (CoT) Experiments and Manual Evaluation of Thought Chains}
    Through our CoT experiments and subsequent human evaluations, we observed that the logic demonstrated by large models often significantly deviates from human rationale, not conforming to conventional human logic. This discrepancy highlights a critical gap in the current AI models' ability to mimic human-like reasoning. Our findings suggest that the instability of large models across different data distributions is partly due to their tendency to latch onto superficial features rather than deeper, more logical structures of reasoning.
In summary, our paper contributes to the field by providing a comprehensive analysis of the reasoning capabilities of large language models. We delve into the nuances of their performance, explore the implications of their learning patterns, and shed light on the discrepancies between AI-driven and human logic. This analytical approach not only enhances our understanding of existing models but also guides the development of more advanced and human-like AI systems.

==> subtexs/voting.tex <==
\begin{figure}[t!]
\centering
%\setlength{\abovecaptionskip}{0.1cm}
%\setlength{\belowcaptionskip}{0.2cm}
\includegraphics[width=0.5\textwidth]{Figures/self-consistency.pdf}
\caption{Self-consistency Evaluation.}
\label{fig:consistency}
\vspace{-1.0em}
\end{figure} 

==> tables/ablation.tex <==
\begin{table}[!t]
\small
\centering
\scalebox{0.75}{
\begin{tabular}{l|c|c|c|c|c }
\hline
\textbf{Dataset} & \textbf{Shuffle 1}  & \textbf{Shuffle 2} & \textbf{Shuffle 3} & {\bf w/ shuffle} & {\bf w/o shuffle}  \\
\hline
LogiQA 2.0  &  {50.52} & 52.28 & 52.55 & 55.34 & 53.23 \\
LogiQA 2.0 zh  & 51.11 & 51.59 & 49.42 & 52.46 & 52.08 \\
ReClor  & 58.96 & 56.32 & 58.24 &60.11 &59.94 \\
AR-LSAT  &  48.29 & 51.47 & 50.76 & 53.42 & 52.44  \\
LogiQA22  & 40.61 & 42.34 & 38.74 & 43.71 & 42.19  \\

\hline
\end{tabular}
}
\caption{\label{Tab:ablation}
Ablation on the shuffle-and-vote method (accuracy \%). }
\vspace{-2em}
\end{table}

==> tables/ablation_bak.tex <==
\begin{table}[!t]
\small
\centering
\scalebox{0.75}{
\begin{tabular}{l|c|c|c|c|c|c }
\toprule
\textbf{Dataset} & \bf Original & \textbf{Shuffle 1}  & \textbf{Shuffle 2} & \textbf{Shuffle 3} & w/ shuffle & w/o shuffle  \\
\hline
LogiQA 2.0 &  52.37 &  {50.52} & 52.28 & 52.55 & 55.34 & 53.23 \\
LogiQA 2.0 zh & 53.18 & 51.11 & 51.59 & 49.42 & 52.46 & 52.08 \\
ReClor & 57.38 & 58.96 & 56.32 & 58.24 &60.11 &59.94 \\
AR-LSAT &  51.49 &  48.29 & 51.47 & 50.76 & 53.42 & 52.44  \\
LogiQA22 & {38.44} & 40.61 & 42.34 & 38.74 & 43.71 & 42.19  \\

\bottomrule
\end{tabular}
}
\caption{\label{Tab:ablation}
Ablation on the shuffle-and-vote method. }
\vspace{-1em}
\end{table}


==> tables/cot.tex <==
\begin{table}[!t]
\small
\centering
\scalebox{0.9}{
\begin{tabular}{l|c|c}
\toprule
\textbf{Model} & \textbf{w/o CoT}  & \textbf{w/ CoT}  \\
\midrule
LLaMA  & 32.34 & 35.05   \\
Falcon  & 32.28 & 34.98   \\
ChatGPT  & 52.10 & 55.75   \\
GPT-4  &  66.34 & 68,47  \\
\bottomrule
\end{tabular}
}
\caption{\label{Tab:cot}
Chain-of-Thought evaluation on GLoRE. All results are in \%. }
\vspace{-2em}
\end{table}

\begin{table}
\centering
\scalebox{0.95}{
\begin{tabular}{l|c|c}
\toprule
     & {\bf CoT correct} & {\bf CoT wrong} \\
\midrule
    {\bf w/o CoT correct} & 65.00 & 1.33 \\
    {\bf w/o CoT wrong} & 3.50 & 30.21 \\
\bottomrule
\end{tabular}
}
\caption{\label{Tab:cot_confusion}
The confusion matrix for GPT-4 results on the LogiQA22 data with/without CoT. All results are in \%.
}
%\vspace{-2em}
\end{table}

==> tables/human-eval.tex <==
\begin{table}[!t]
\small
\centering
\scalebox{0.8}{
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Coherence}  & \textbf{Completeness} & \textbf{Correctness} & {\bf Relevance}  \\
\midrule
\textbf{LLaMA}  &  3.38 & 3.53 & 3.00 & 4.50  \\
\textbf{Falcon}  &3.21 & 3.44 & 3.15 & 4.50  \\
\textbf{ChatGPT}  & 4.00 & 4.81 & 3.76 & 4.72  \\
\textbf{GPT-4}  &  4.52 & 4.81 & 4.51 & 4.89  \\

\bottomrule
\end{tabular}
}
\caption{\label{Tab:human}
Human evaluation of CoT generations. }
\vspace{-2em}
\end{table}

==> tables/manual.tex <==
\begin{table}[!t]
\small
\centering
\scalebox{1}{
\begin{tabular}{lcl}
\toprule
\textbf{Dataset} & \bf API Result & \textbf{Chat UI Result }  \\
\midrule
LogiQA 2.0 test &  72.25 &  {\bf 75.26} (73/97) \\
LogiQA 2.0 zh test & {\bf 70.56} & 60.95 (64/105) \\
ReClor dev & 87.20 & {\bf 92.00} (92/100) \\
AR-LSAT test &  73.12 & {\bf 83.65} (87/104) \\
LogiQA22 & {\bf 58.49} & 50.67 (76/150)  \\
\midrule
ConTRoL & 56.40  & {\bf 58.18} (64/110) \\
HELP & 46.01 & {\bf 53.33} (56/105) \\
TaxiNLI test & 60.08 & {\bf 75.47} (80/106) \\
NaN-NLI & 76.74 & {\bf 71.00} (71/100) \\
\midrule
FraCas & 75.35 & {\bf 76.25} (61/80) \\
RuleTaker dev & {\bf 60.19} & 59.09 (65/110) \\
ProofWriter dev& {\bf 59.66} & 54.00 (54/100) \\
\bottomrule
\end{tabular}
}
\caption{\label{Tab:manual}
GPT-4 manual tests from Chat UI (accuracy \%). The numbers in brackets denote the number of correct samples and total tested samples. }
%\vspace{-2em}
\end{table}


==> tables/probing.tex <==
\begin{table}[!t]
\small
\centering
\scalebox{1}{
\begin{tabular}{lcc}
\toprule
\textbf{Dataset} & \textbf{Single Model} & \textbf{Voting  Model}  \\
\midrule
LogiQA 2.0  & 52.37 & \bf 54.58 \\
LogiQA 2.0 zh  & \bf 53.18 &  52.01 \\
ReClor   & 57.38  & \bf 59.00 \\
AR-LSAT  &  51.49 &  \bf 53.91 \\
LogiQA22 & 38.44 & \bf 41.14 \\
\bottomrule
\end{tabular}
}
\caption{\label{Tab:probing}
ChatGPT results with self-consistency voting. 
}
%\vspace{-1em}
\end{table}

==> tables/tuned.tex <==
\begin{table}
\small
\centering
\scalebox{1}{
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Dataset} & \textbf{7b-base} & \textbf{Alpaca} & \textbf{7b-tuned} \\
\midrule
LogiQA 2.0 test & 18.04  & 22.99 & \bf 52.74\\
LogiQA 2.0 zh test & 19.06  & 22.54 & \bf 31.18\\
ReClor dev & 15.83  & 22.38 & \bf 55.20\\
AR-LSAT test & 13.91 & 13.16 & \bf 21.43 \\
LogiQA22 & 20.25  & 21.16 & \bf 35.16\\

\bottomrule
\end{tabular}
}
\caption{\label{Tab:finetune}
Fine-tune LLaMA on the LogiQA dataset (accuracy \%). ``7b-base'' is the base model of LLaMA-7b; ``Alpaca'' is an instruction-tuned LLaMA-7b with GPT-4 Alpaca data; ``7b-tuned'' is our fine-tuned LLaMA-7b on the LogiQA 2.0 training set. All results are in \%.}
\vspace{-3em}
\end{table}

==> tables/types.tex <==
\begin{table*}
\small
\centering
\scalebox{0.83}{
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Types} & \textbf{ChatGPT} & \textbf{GPT-4} & \textbf{LLaMA} & \textbf{Falcon} \\
%\hline
%\textbf{\# instances} & 150 & 150 \\
\midrule
Categorical reasoning &  83.83\% (389/464) & 95.04\% (441/464) & 22.84\% (106/464) & 20.91\% (97/464)\\
Sufficient condition reasoning & 44.99\% (175/389) & 63.75\% (248/389) & 20.82\% (81/389) & 20.56\% (80/389)\\
Necessary condition reasoning & 37.46\% (124/331) & 60.73\% (201/331) & 19.64\% (65/331) & 25.38\% (84/331) \\
Conjunctive reasoning & 26.79\% (75/280) & 35.00\% (98/280)  & 7.86\% (22/280) & 12.86\% (36/280)\\
Disjunctive reasoning & 15.75\% (60/381) & 27.03\% (103/381) & 7.87\% (30/381) & 17.85\% (68/381)\\
\bottomrule
\end{tabular}
}
\caption{\label{Tab:types}
LLMs' performance across reasoning types (accuracy \%).
}
\vspace{-2em}
\end{table*}
